Diversity in Software Engineering Education: Exploring Motivations, Influences, and Role Models Among Undergraduate Students

Software engineering (SE) faces significant diversity challenges in both academia and industry, with underrepresented students encountering hostile environments, limited representation, and systemic biases that hinder their academic and professional success. Despite significant research on the exclusion experienced by students from underrepresented groups in SE education, there is limited understanding of the specific motivations, influences, and role models that drive underrepresented students to pursue and persist in the field. This study explores the motivations and influences shaping the career aspirations of students from underrepresented groups in SE, and it investigates how role models and mentorship impact their decisions to stay in the field. We conducted a cross-sectional survey with undergraduate SE students and related fields, focusing on their motivations, influences, and the impact of mentorship and role models on their career paths. We identified eight motivations for pursuing SE, with career advancement, technological enthusiasm, and personal growth being the most common. Family members, tech influencers, teachers, and friends were key influences, though 64\% of students reported no specific individual influence. Role models, particularly tech influencers and family members play a critical role in sustaining interest in the field, especially for underrepresented groups. This study provides insights into the varied motivations and influences that guide underrepresented students' decisions to pursue SE. It emphasizes the importance of role models and highlights the need for intersectional approaches to better support diversity in the field.

==> tables/smells_discussion.tex <==
\begin{table}[h!]
\centering
\label{tab:smells}
\caption{Summary of Characteristics, Debt, and Common Examples of Smells}
\begin{tabular}{|m{1.5cm}|m{3.2cm}|m{2.7cm}|}
\hline
\textbf{Smell} & \textbf{Characteristic} & \textbf{Common Examples} \\ \hline
\textbf{Code Smells} & Technical issues, such as complex code patterns and design flaws. Complicate future maintenance and readability. Related to technical debt. & Duplicate code, Dead code, Long parameter list, Data clumps, Long functions, Primitive obsession, Large class, Shotgun surgery. \\ \hline
\textbf{Community Smells} & Social and organizational issues. Derived from poor socio-technical decisions. Affects team dynamics and communication, leading to reduced productivity. Related to social debt. & Black cloud, Cognitive distance, DevOps clash, Dispersion, Dissensus, Informality excess, Architecture by osmosis, Power distance, Organizational silo. \\ \hline
\textbf{Bias Smells} & Bias-related issues. Impact both technical performance and fairness, revealing deficiencies in design and team diversity, leading to biased outcomes. Related to fairness debt. & Context oversimplification, Data imbalance, Metrics inadequacies, Ad-hoc testing, Individual diversity unawareness, Non-diverse team. \\ \hline
\end{tabular}
\end{table}
